DUALZ: Deep UNCOVER-ALMA Legacy High-Z Survey

We present the survey design and initial results of the ALMA Cycle 9 program of DUALZ, which aims to establish a joint ALMA and JWST public legacy field targeting the massive galaxy cluster Abell 2744. DUALZ features a contiguous $4'\times6'$ ALMA 30-GHz-wide mosaic in Band 6, covering areas of $\mu>2$ down to a sensitivity of $\sigma=32.7~\mu$Jy. Through a blind search, we identified 69 dust continuum sources at S/N $\gtrsim5.0$ with median redshift and intrinsic 1.2-mm flux of $z=2.30$ and $S_{\rm 1.2mm}^{\rm int}=0.24$~mJy. Of these, 27 have been spectroscopically confirmed, leveraged by the latest NIRSpec observations, while photometric redshift estimates are constrained by the comprehensive HST, NIRCam, and ALMA data for the remaining sources. With priors, we further identify a [CII]158 $\mu$m line emitter at $z=6.3254\pm0.0004$, confirmed by the latest NIRSpec spectroscopy. The NIRCam counterparts of the 1.2-mm continuum exhibit undisturbed morphologies, denoted either by disk or spheroid, implying the triggers for the faint mm emission are less catastrophic than mergers. We have identified 8 HST-dark galaxies (F150W$>$27mag, F150W$-$F444W$>$2.3) and 2 JWST-dark (F444W$>$30mag) galaxy candidates among the ALMA continuum sources. The former includes face-on disk galaxies, hinting that substantial dust obscuration does not always result from inclination. We also detect a marginal dust emission from an X-ray-detected galaxy at $z_{\rm spec}=10.07$, suggesting an active co-evolution of the central black hole and its host. We assess the infrared luminosity function up to $z\sim10$ and find it consistent with predictions from galaxy formation models. To foster diverse scientific outcomes from the community, we publicly release reduced ALMA mosaic maps, cubes, and the source catalog.

==> latexdefs.tex <==
\def\farcm{% 
 \mbox{.\kern -0.7ex\raisebox{.9ex}{\scriptsize$\prime$}}% 
}% 
\def\farcs{% 
 \mbox{% 
  \kern  0.13ex.% 
  \kern -0.95ex\arcsec% 
  \kern -0.1ex% 
 }% 
}% 
%\renewcommand\case[2]{\mbox{$\frac{#1}{#2}$}}% 
%\renewcommand\slantfrac{\case}% 
\newcommand\onehalf{\slantfrac{1}{2}}% 
\newcommand\onethird{\slantfrac{1}{3}}% 
\newcommand\twothirds{\slantfrac{2}{3}}% 
\newcommand\onequarter{\slantfrac{1}{4}}% 
\newcommand\threequarters{\slantfrac{3}{4}}% 
\newcommand\ubvr{\mbox{$U\!BV\!R$}}%% UBVR system 
\newcommand\ub{\mbox{$U\!-\!B$}}%   % U-B 
\newcommand\bv{\mbox{$B\!-\!V$}}%   % B-V 
%\renewcommand\vr{\mbox{$V\!-\!R$}}%   % V-R 
\newcommand\ur{\mbox{$U\!-\!R$}}%   % U-R 
\makeatletter
\newcommand\ion[2]{#1$\;$\protect \textsmaller{\rmfamily\@Roman{#2}}}% 
\newcommand\smion[2]{#1$\;$\protect \footnotesize{\rmfamily\@Roman{#2}}\small}% 
\newcommand\scion[2]{#1$\;$\protect \tiny{\rmfamily\@Roman{#2}}\scriptsize}% 
\makeatother
\newcommand\nodata{ ~$\cdots$~ }% 
\newcommand\diameter{\ooalign{\hfil/\hfil\crcr\mathhexbox20D}}% 
\newcommand\degr{\arcdeg}% 
\newcommand\Sun{\sun}% 
\newcommand\Sol{\sun}% 
\newcommand\sun{\odot}% 
\newcommand\Mercury{\astro{\char1}}% Mercury symbol, "1" 
\newcommand\Venus{\astro{\char2}}% Venus symbol, "2" 
\newcommand\Earth{\earth}% 
\newcommand\Terra{\earth}% 
\newcommand\earth{\oplus}% 
\newcommand\Mars{\astro{\char4}}% Mars symbol, "4" 
\newcommand\Jupiter{\astro{\char5}}% Jupiter symbol, "5" 
\newcommand\Saturn{\astro{\char6}}% Saturn symbol, "6" 
\newcommand\Uranus{\astro{\char7}}% Uranus symbol, "7" 
\newcommand\Neptune{\astro{\char8}}% Neptune symbol, "8" 
\newcommand\Pluto{\astro{\char9}}% Pluo symbol, "9" 
\newcommand\Moon{\astro{\char10}}% Moon symbol, "M" 
\newcommand\Luna{\Moon}% 
\newcommand\Aries{\astro{\char11}}% 
\newcommand\VEq{\Aries}% vernal equinox (Aries) 
\newcommand\Taurus{\astro{\char12}}% 
\newcommand\Gemini{\astro{\char13}}% 
\newcommand\Cancer{\astro{\char14}}% 
\newcommand\Leo{\astro{\char15}}% 
\newcommand\Virgo{\astro{\char16}}% 
\newcommand\Libra{\astro{\char17}}% 
\newcommand\AEq{\Libra}% autumnal equinox (Libra) 
\newcommand\Scorpius{\astro{\char18}}% 
\newcommand\Sagittarius{\astro{\char19}}% 
\newcommand\Capricornus{\astro{\char20}}% 
\newcommand\Aquarius{\astro{\char21}}% 
\newcommand\Pisces{\astro{\char22}}% 

\newcommand\caii{Ca~{\sc ii}}
\newcommand\mgi{Mg~{\sc i}}
\newcommand\fehphot{$\rm{[Fe/H]_{phot}}$}
\newcommand\fehspec{$\rm{[Fe/H]_{spec}}$}
\newcommand\lcdm{$\Lambda$CDM}
\newcommand{\teff}{$T_{\rm{eff}}$}
\newcommand{\mathteff}{T_{\rm{eff}}}
\newcommand{\logg}{$\log g$}
\newcommand{\mathlogg}{\log g}
\newcommand{\feh}{[Fe/H]}
\newcommand{\mathfeh}{\rm{[Fe/H]}}
\newcommand{\afe}{[$\alpha$/Fe]}
\newcommand{\xfe}{[X/Fe]}
\newcommand{\mathafe}{\rm{[\alpha/Fe]}}
\newcommand{\mathxfe}{\rm{[X/Fe]}}
\newcommand{\ah}{[$\alpha$/H]}
\newcommand{\mathah}{\rm{[\alpha/H]}}
\newcommand{\vt}{$v_t$}
\newcommand{\mathvt}{v_t}
\newcommand{\cfht}{\textsc{cfht}}
\newcommand{\ha}{H$\alpha$}
\newcommand{\deep}{\textsc{deep2}}
\newcommand{\deimos}{\textsc{deimos}}
\newcommand{\mathaa}{\mathrm{\AA}}
\newcommand{\ngcaf}{NGC~1904 (M79)}
\newcommand{\ngca}{M79}
\newcommand{\ngcb}{NGC 2419}
\newcommand{\ngccf}{NGC~6205 (M13)}
\newcommand{\ngcc}{M13}
\newcommand{\ngcdf}{NGC~6838 (M71)}
\newcommand{\ngcd}{M71}
\newcommand{\ngce}{NGC 7006}
\newcommand{\ngcff}{NGC~7078 (M15)}
\newcommand{\ngcf}{M15}
\newcommand{\ngcg}{NGC 7492}
\newcommand{\bd}{BD+28$^{\circ}$~4211}

\newcommand{\otoprule}{\midrule[\heavyrulewidth]}

\newcommand\bain{Bull.~Astron.~Inst.~Netherlands}
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{Fund.~Cosmic~Phys.}
          % Fundamental Cosmic Physics
\newcommand\gca{Geochim.~Cosmochim.~Acta}
          % Geochimica Cosmochimica Acta
\newcommand\grl{Geophys.~Res.~Lett.}
          % Geophysics Research Letters
\newcommand\jcp{J.~Chem.~Phys.}
          % Journal of Chemical Physics
\newcommand\jgr{J.~Geophys.~Res.}
          % Journal of Geophysical Research
\newcommand\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{Mem.~Soc.~Astron.~Italiana}
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{Nucl.~Phys.~A}
          % Nuclear Physics A
\newcommand\physrep{Phys.~Rep.}
          % Physics Reports
\newcommand\physscr{Phys.~Scr}
          % Physica Scripta
\newcommand\planss{Planet.~Space~Sci.}
          % Planetary Space Science
\newcommand\procspie{Proc.~SPIE}
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

